Two cycle-chord graphs are $e$-positive

We prove Gebhard and Sagan's $(e)$-positivity of the line graphs of tadpoles in noncommuting variables. This implies the $e$-positivity of these line graphs. We then extend this $(e)$-positivity result to that of certain cycle-chord graphs, and derive the bivariate generating function of all cycle-chord graphs.

==> tadpoleLtadpole.tex <==
% !TEX root = csf2.tex

\coordinate (0) at (3, 0);
\coordinate (1) at (11.5, 0);
\coordinate (2) at (9.5, 0);
\coordinate (l) at (5, 0);
\coordinate (3) at (2.37, 1.9);
\coordinate (4) at (0.56, 2.9); 
\coordinate (5) at (-1.56, 2.56); 
\coordinate (6) at (-2.8, 1);
\coordinate (7) at (-2.8, -1);
\coordinate (8) at (-1.56, -2.56);
\coordinate (9) at (0.56, -2.9);
\coordinate (10) at (2.37, -1.9);
\coordinate (a) at (6.9, 0);
\coordinate (b) at (7.3, 0); 
\coordinate (c) at (7.7, 0);
\coordinate (d) at (-2.95, .5);
\coordinate (e) at (-3, 0); 
\coordinate (f) at (-2.95, -.5);
\draw[edge] (1)--(2)--(8, 0) (6.6, 0)--(l)--(0);  
\draw[edge] (-2.8, 1.1) arc [start angle=160, end angle=-160, radius=3cm]; 
\foreach \e in {1,2,l}
  \shade[ball](\e) circle(.6);
\foreach \e in {3,...,5,8,9,10}
  \shade[ball](\e) circle(.6);
\shade[ball](0) circle(.6);
\foreach \e in {a, b, c, d, e, f}
  \shade[apball](\e) circle(.08);

\begin{scope}[xshift=19cm, rotate=90]
\coordinate (v) at (-.92, -2.85);
\coordinate (u) at (.92, -2.85);
\coordinate (m-1) at (2.42, -1.76);
\coordinate (m-2) at (3, 0);
\coordinate (m-3) at (2.42, 1.76);
\coordinate (a) at (.6, 2.95);
\coordinate (b) at (0, 3);
\coordinate (c) at (-.6, 2.95);
\coordinate (-3) at (-2.42, 1.76);
\coordinate (-2) at (-3, 0);
\coordinate (-1) at (-2.43, -1.76);
\coordinate (w) at (0, -4.6-.7);
\coordinate (l-1) at (0, -6.5-.9);
\coordinate (d) at (0, -8.5-1.2);
\coordinate (e) at (0, -9.1-1.2);
\coordinate (f) at (0, -9.7-1.2);
\coordinate (2) at (0, -11.7-1.2);
\coordinate (1) at (0, -13.7-1.2);
\draw[edge]
(u)--(w)--(v)
(w)--(l-1)--(0, -9.2) 
(0, -10.2-1.2)--(2)--(1);
\draw[edge] (1, 2.85) arc [start angle=70, end angle=-250, radius=3cm]; 
\foreach \e in {l-1, 2, 1}
  \shade[ball](\e) circle(.6);
\foreach \f in {m-1, m-2, m-3, -3, -2, -1}
  \shade[ball](\f) circle(.6);
\foreach \h in {u, v, w}
 \shade[ball](\h) circle(.6);
%  node{$\h$}; 
\foreach \g in {a, b, c, d, e, f}
  \shade[apball](\g) circle(.08);
\draw(1, -4.3);
% node{$e_1$};
\draw(-1, -4.3);
%node{$e_2$};
\end{scope}
